Mix Forcing: Causal Pre-Training via Mixture Attention for Interactive World Models

While interactive video world models require autoregressive generation, directly adapting pretrained bidirectional video diffusion models into autoregressive ones with teacher forcing can disrupt their visual priors and degrade autoregressive generation quality. In this paper, we introduce Mix Forcing, a causal pre-training paradigm for interactive video world models, implemented with the Mixture-of-Bidirectional-and-Autoregressive (MoBA) attention. Mix Forcing jointly trains a video diffusion model with both teacher forcing and bidirectional training, yielding a strong causal initialization for few-step post-training. In self-attention, Mix Forcing leverages teacher forcing to learn causal next-chunk prediction for autoregressive rollout, while using bidirectional attention to preserve pretrained visual priors. To support online text interaction, Mix Forcing further adopts a chunk-wise cross-attention design that conditions each video chunk on a shared environment prompt and its own local prompt, without exposing future instructions to the current chunk. Following causal pre-training on a 14B image-to-video model, we apply consistency and distribution matching distillation to obtain a four-step autoregressive generator. Experiments on our internal benchmark and public benchmarks, including WBench and SANA-WM-Bench, show that our model achieves state-of-the-art visual quality and timely event following with precise camera control. Notably, our model supports high-fidelity long-horizon generation without quality degradation even over one-hour rollouts. Project page is here: https://zelingao98.github.io/mixforcing

==> combined_layout.tex <==
\makeatletter
\newcommand{\mixforcingsupplementarylayout}{%
  \RemoveFromHook{env/figure/begin}[main-layout]%
  \RemoveFromHook{env/figure*/begin}[main-layout]%
  \RemoveFromHook{env/wrapfigure/begin}[main-layout]%
  \RemoveFromHook{env/table/begin}[main-layout]%
  \RemoveFromHook{env/table*/begin}[main-layout]%
  \RemoveFromHook{env/table/end}[main-layout]%
  \RemoveFromHook{env/table*/end}[main-layout]%
  \setlength{\parskip}{6pt}%
  \renewcommand{\paragraph}{%
    \@startsection{paragraph}{4}{\z@}%
      {0.5ex plus 0.2ex minus 0.1ex}{-1em}%
      {\normalfont\normalsize\bfseries}}%
  \setlength{\@fptop}{0pt}%
  \setlength{\@fpbot}{0pt plus 1fil}%
  \raggedbottom
  \setcounter{topnumber}{2}\setcounter{bottomnumber}{1}\setcounter{totalnumber}{3}%
  \renewcommand{\floatpagefraction}{0.5}%
  \setlength{\textfloatsep}{12pt plus 2pt minus 2pt}%
  \setlength{\floatsep}{10pt plus 2pt minus 2pt}%
  \setlength{\intextsep}{8pt plus 2pt minus 2pt}%
  \setcounter{figure}{0}\setcounter{table}{0}\setcounter{equation}{0}%
  \renewcommand{\thefigure}{S\arabic{figure}}%
  \renewcommand{\thetable}{S\arabic{table}}%
  \renewcommand{\theequation}{S\arabic{equation}}%
  \renewcommand{\theHfigure}{supp.\arabic{figure}}%
  \renewcommand{\theHtable}{supp.\arabic{table}}%
  \renewcommand{\theHequation}{supp.\arabic{equation}}%
  \AddToHook{env/figure/begin}[supp-layout]{%
    \setlength{\abovecaptionskip}{4pt}%
    \setlength{\belowcaptionskip}{0pt}}%
  \AddToHook{env/table/begin}[supp-layout]{%
    \setlength{\abovecaptionskip}{0pt}%
    \setlength{\belowcaptionskip}{4pt}}%
}
\makeatother


==> public_style.tex <==
\usepackage{etoolbox}
\iclrfinalcopy

\renewcommand{\rmdefault}{EBGaramond-LF}
\normalfont
\urlstyle{same}

\addtolength{\topmargin}{12pt}
\setlength{\headsep}{16pt}

\makeatletter
\patchcmd{\@maketitle}{\LARGE\sc \@title\par}%
  {\LARGE\fontfamily{EBGaramond-LF}\scshape\raggedright\hyphenpenalty=10000 \@title\par}{}%
  {\PackageError{public-style}{Title font patch failed}{Check the original title definition.}}
\patchcmd{\@maketitle}{\lhead{Published as a conference paper at ICLR 2027}}{}{}%
  {\PackageError{public-style}{Header patch failed}{Check the original title definition.}}
\patchcmd{\@maketitle}
  {\begin{tabular}[t]{l}\bf\rule{\z@}{24pt}\@author\end{tabular}}%
  {\vskip 19pt {\centering\normalfont\normalsize\@author\par}}{}%
  {\PackageError{public-style}{Author patch failed}{Check the original title definition.}}
\patchcmd{\@maketitle}{\vskip 0.3in minus 0.1in}{\vskip 7pt}{}{}
\makeatother
\fancyhead{}
\fancyhead[L]{\small Mix Forcing: Causal Pre-Training for Interactive World Models}
\fancypagestyle{publictitle}{%
  \fancyhead{}%
  \fancyhead[L]{\normalsize\bfseries Xu Lab}%
  \fancyhead[R]{\normalsize\itshape HKUST}%
}
\AddToHook{cmd/maketitle/after}{\thispagestyle{publictitle}}

\usepackage{tcolorbox}
\definecolor{abstractbg}{HTML}{F7F2F3}
\renewenvironment{abstract}{\begin{tcolorbox}[
  colback=abstractbg,colframe=white,boxrule=0pt,arc=10pt,
  left=16pt,right=16pt,top=10pt,bottom=11pt,width=\textwidth,
  enlarge left by=0mm,before skip=22pt,after skip=10pt]
  {\centering\normalfont\large\bfseries\abstractname\par}\nobreak\vspace{3pt}%
  \noindent\ignorespaces}{\end{tcolorbox}}

